The AMIGA sample of isolated galaxies -- Effects of Environment on Angular momentum

We investigate the relationship between the baryonic angular momentum and mass for a sample of 36 isolated disc galaxies with resolved HI kinematics and infrared WISE photometry drawn from -- and representative in terms of morphologies, stellar masses and HI-to-star fraction of -- the carefully-constructed AMIGA sample of isolated galaxies. Similarly to previous studies performed on non-isolated galaxies, we find that the relation is well described by a power law $j_{bar} \propto M_{bar}^\alpha$. We also find a slope of $\alpha = 0.54 \pm 0.08$ for the AMIGA galaxies, in line with previous studies in the literature; however, we find that the specific angular momenta of the AMIGA galaxies are on average higher than those of non-isolated galaxies in the literature. This is consistent with theories stipulating that environmental processes involving galaxy-galaxy interaction are able to impact the angular momentum content of galaxies. However, no correlation was found between the angular momentum and the degree of isolation, suggesting that there may exist a threshold local number density beyond which the effects of the environment on the angular momentum become important.

==> list-sources.tex <==
\begin{table}
{\scriptsize
\centering
\begin{tabular}{l c c c c}
\hline
\hline
CIG ID & Tel. & $\theta_{\rm maj} \times \theta_{\rm min}\,('')$ & $\theta_{\rm PA}$ & Ref. \\ 
\hline
85 & GMRT & 22.6 $\times$ 18.8 & 24.2 & \citet{Sengupta2012} \\ 
96 & VLA C+D & 16.8 $\times$ 15.6 & -30.1 & \citet{Ramirez-Moreta2018} \\ 
102 & WSRT & 29.5 $\times$ 24.5 & 0.0 & WHISP $^a$ \\ 
103 & VLA & 52.9 $\times$ 45.5 & 8.7 & VLA archive \\ 
123 & VLA C+D & 17.6 $\times$ 15.7 & -34.4 & VLA archive \\ 
134 & VLA D & 68.1 $\times$ 52.5 & 24.6 & VLA archive \\ 
147 & WSRT & 33.1 $\times$ 23.5 & 0.0 & WHISP $^a$ \\ 
159 & WSRT & 29.7 $\times$ 23.0 & 0.0 & WHISP $^a$ \\ 
188 & GMRT & 43.1 $\times$ 36.6 & -22.1 & \citet{Sengupta2012} \\ 
232 & WSRT & 32.9 $\times$ 19.6 & 0.0 & WHISP $^a$ \\ 
240 & VLA D & 62.1 $\times$ 54.4 & -56.8 & VLA archive \\ 
292 & VLA & 46.6 $\times$ 42.1 & -42.3 & \citet{Portas2011} \\ 
314 & WSRT & 28.0 $\times$ 27.7 & 0.0 & WHISP $^a$ \\ 
329 & VLA & 13.9 $\times$ 13.5 & -22.8 & \citet{Spekkens2006} \\ 
359 & VLA & 65.9 $\times$ 60.8 & -12.42 & VLA archive \\ 
361 & VLA & 16.3 $\times$ 13.5 & -87.1 & \citet{Spekkens2006} \\ 
421 & VLA & 56.3 $\times$ 50.0 & 44.7 & \citet{Espada2006} \\ 
463 & VLA & 45.6 $\times$ 42.5 & 75.1 & \citet{Espada2006} \\ 
512 & GMRT & 17.3 $\times$ 13.3 & -49.6 & \citet{Sengupta2012} \\ 
551 & VLA & 47.6 $\times$ 43.1 & 58.6 & \citet{Espada2006} \\ 
553 & Apertif & 25.2 $\times$ 12.8 & 2.2 & Apertif $^b$ \\ 
571 & VLA & 67.2 $\times$ 52.3 & 18.1 & VLA archive \\ 
581 & Apertif & 30.8 $\times$ 14.5 & -2.3 & Apertif $^b$ \\ 
587 & Apertif & 25.1 $\times$ 17.9 & -3.1 & Apertif $^{b,c}$ \\ 
604 & WSRT & 33.2 $\times$ 28.7 & 0.0 & WHISP $^a$ \\ 
616 & VLA D & 64.5 $\times$ 58.1 & -15.6 & VLA archive \\ 
626 & GMRT & 30.0 $\times$ 30.0 & 45.0 & \citet{Ponomareva2016} \\ 
660 & VLA D & 58.8 $\times$ 46.3 & 66.6 & VLA archive \\ 
676 & Apertif & 17.3 $\times$ 13.2 & 0.0 & Apertif $^b$ \\ 
736 & VLA D & 58.0 $\times$ 52.2 & 81.7 & VLA archive \\ 
744 & VLA D & 67.2 $\times$ 55.7 & 74.7 & VLA archive \\ 
812 & VLA & 53.7 $\times$ 46.5 & 65.5 & \citet{Espada2006} $^c$ \\ 
983 & Apertif & 24.5 $\times$ 13.6 & -1.7 & Apertif $^b$ \\ 
988 & Apertif & 29.7 $\times$ 13.4 & 1.5 & Apertif $^b$ \\ 
1000 & Apertif & 23.5 $\times$ 13.5 & -1.6 & Apertif $^b$ \\ 
1004 & VLA D & 130.0 $\times$ 48.9 & 1.7 & VLA archive \\ 
1006 & Apertif & 25.0 $\times$ 14.0 & 0.5 & Apertif $^b$ \\ 
1019 & VLA D & 56.4 $\times$ 47.9 & 8.7 & VLA archive \\ 
\hline
\end{tabular}\\
$^a$ Data from the WHISP survey \citep{Swaters2002};
$^b$ Data from the Apertif DR1 \citep{Adams2022};
$^c$ Galaxy excluded from the $j$-sample because of a non-detection in the {\it WISE} bands.
\caption{Properties of the \hi\ data for galaxies in the AMIGA angular momentum sample.}\label{tb:sources}}
\end{table}

